A Stitch in Time Saves Nine: Detecting and Mitigating Hallucinations of LLMs by Validating Low-Confidence Generation

Recently developed large language models have achieved remarkable success in generating fluent and coherent text. However, these models often tend to 'hallucinate' which critically hampers their reliability. In this work, we address this crucial problem and propose an approach that actively detects and mitigates hallucinations during the generation process. Specifically, we first identify the candidates of potential hallucination leveraging the model's logit output values, check their correctness through a validation procedure, mitigate the detected hallucinations, and then continue with the generation process. Through extensive experiments with GPT-3.5 (text-davinci-003) on the 'article generation task', we first demonstrate the individual efficacy of our detection and mitigation techniques. Specifically, the detection technique achieves a recall of ~88% and the mitigation technique successfully mitigates 57.6% of the correctly detected hallucinations. Importantly, our mitigation technique does not introduce new hallucinations even in the case of incorrectly detected hallucinations, i.e., false positives. Then, we show that the proposed active detection and mitigation approach successfully reduces the hallucinations of the GPT-3.5 model from 47.5% to 14.5% on average. We further demonstrate the effectiveness and wide applicability of our approach through additional studies including performance on different types of questions (multi-hop and false premise questions) and with another LLM from a different model family (Vicuna). In summary, our work contributes to improving the reliability and trustworthiness of large language models, a crucial step en route to enabling their widespread adoption in real-world applications.

==> Tables/data/data_examples.tex <==
\begin{table*}[]
\centering
% \small
\resizebox{0.98\linewidth}{!}
{
\begin{tabular}{l|l}
\toprule

  \textbf{Domain} & \textbf{Examples} \\ 
  \midrule
 \textbf{Sports} & Rick Mahler, Akila Dananjaya, Steven Threet, Paul Caddis, Brian Petrovek, Dan Stearns\\
 % , Malcolm Brogdon\\
 \textbf{Politics} & Lee Hsien Loong, C. V. Ananda Bose, Anthony Dimond, Robert F. Kennedy, John Cushnahan \\
 % , Roy Beggs Jr.\\
 \textbf{Music} & Dawn Landes, Rise Pantheon Dreams, Rod Morgenstein, Fat Wreck Chords, Martina Sorbara\\
 % Seyi Shay
 % Torry Castellano 
 % Jerry Leger
 % Pino Palladino

 \textbf{Films \& TV} & Marshall Manesh, Linda Hunt, Wayne Allyn Root, Lindsay Crouse, Evan Rachel Wood\\
 % , Tristan Rogers\\
 \textbf{Literature} & Eleanor Arnason, Frank Abagnale Jr., Adiele Afigbo, Hope Cooke, Vitaliano Brancati\\
 % Saul David
 \textbf{Science} & John Russell Reynolds, Don R. Swanson, Jearl Walker, Thomas Harriot\\
  \textbf{Defense} & Eden Natan-Zada, George Milne, Modibo Adama, William J. Flanagan, Jr.\\
 \textbf{Arts} & Johan Christian Dahl, Twila Shively, Philippe Dodard, Adja Yunkers, Nigel Milsom\\
 \textbf{Others} & Frederick Thomas Brentnall,  Murray G. Ross, Nate Saint, Tomasz Lis, Robert Holgate\\
 % Yaakov Israel Ifargan, , \\
 \bottomrule
\end{tabular}
}
  \caption{Examples of topics from different domains.}
  \label{tab:data_examples}
\end{table*}

==> Tables/data/stats_type1.tex <==

\begin{table}[]
\centering
% \small
% \resizebox{0.98\linewidth}{!}
{
\begin{tabular}{l|l}
\toprule

  \textbf{Domain} & \textbf{\# Instances} \\ 
  \midrule
 \textbf{Sports} & \\
 \textbf{Films \& TV} & \\
 \textbf{Music} & \\
 \textbf{Literature} & \\
 \textbf{Defense} & \\
 \textbf{Science} & \\
 \textbf{Business} & \\
 \textbf{Politics} & \\
 \midrule
 \textbf{Total} & \\
\bottomrule
\end{tabular}
}
  \caption{Distribution of instances in different domains for Type 1 evaluation data.}
  \label{tab:stats_type_1}
\end{table}

==> Tables/detection/keyword_level_detection_accuracy.tex <==
\begin{table}[]
\centering
\small
\resizebox{0.98\linewidth}{!}
{
\begin{tabular}{l|l|llll}
\toprule
\textbf{Method} & \textbf{Accuracy} & \multicolumn{2}{c}{\textbf{Hallucinated}} & \multicolumn{2}{c}{\textbf{Not Hallucinated}} \\ 

& & \textbf{Prec.} & \textbf{Rec.} & \textbf{Prec.} & \textbf{Rec.} \\
\midrule

\textbf{Self-Inquiry} & 0.659 & 53.85 & 50.00 & 72.24 & 75.23 \\

\textbf{Web-Search} & \textbf{0.761} & {61.87} & {90.86} & {92.75} & 67.73 \\

\bottomrule
\end{tabular}
}
  \caption{Comparing hallucination detection accuracy (\textbf{at keyword level}) of self-inquiry and web-search techniques. It also shows individual precision and recall on both hallucinated and not hallucinated instances.}
  \label{tab:keyword_level_detection_accuracy_self_inquiery_vs_web_search}
\end{table}

==> Tables/hallucination_causes_further_hallucination/conditional_probabilities_hallucination.tex <==

% \begin{table*}[]
%     \begin{subtable}{\linewidth}
%       \centering
%         \caption{}
%         % \begin{tabular}{ll}
%         %     1 & 2
%         % \end{tabular}
%         \begin{tabular}{l|l}
%         \toprule
%         P ($S_2$ is Hallu. | $S_1$ is Hallu.) & P ($S_2$ is not Hallu. | $S_1$ is Hallu.) \\
%         \midrule
%         83.33\%                         & 16.67\%               \\
%         \bottomrule
%         \end{tabular}
%     \end{subtable}%
    
%     \begin{subtable}{\linewidth}
%       \centering
%         \caption{}
%         \begin{tabular}{l|l}
%         \toprule
%         P ($S_3$ is Hallu. | $S_2$ v $S_1$ is Hallu.) & P ($S_3$ is not Hallu. | $S_2$ v $S_1$ is Hallu.) \\
%         \midrule
%         83.33\%                         & 16.67\%               \\
%         \bottomrule
%         \end{tabular}
%     \end{subtable} 

%     \begin{subtable}{\linewidth}
%       \centering
%         \caption{}
%         \begin{tabular}{l|l}
%         \toprule
%         P ($S_4$ is Hallu. | $S_3$ v $S_2$ v $S_1$ is Hallu.) & P ($S_5$ is not Hallu. | $S_3$ v $S_2$ v $S_1$ is Hallu.) \\
%         \midrule
%         83.33\%                         & 16.67\%               \\
%         \bottomrule
%         \end{tabular}
%     \end{subtable} 
    
%     \begin{subtable}{\linewidth}
%       \centering
%         \caption{}
%         \begin{tabular}{l|l}
%         \toprule
%         P ($S_5$ is Hallu. | $S_4$ v $S_3$ v $S_2$ v $S_1$ is Hallu.) & P ($S_5$ is not Hallu. | $S_4$ v $S_3$ v $S_2$ v $S_1$ is Hallu.) \\
%         \midrule
%         83.33\%                         & 16.67\%               \\
%         \bottomrule
%         \end{tabular}
%     \end{subtable} 
%     \caption{Global caption}
    
% \end{table*}


\begin{table}[]
\centering
\small
\resizebox{0.98\linewidth}{!}
{
\begin{tabular}{l|l|l|l|l}
\toprule
 &  $\mathbf{S_2}$ & $\mathbf{S_3}$ & $\mathbf{S_4}$ & $\mathbf{S_5}$\\ \midrule
 \% Hallucinations & - & - & - & -  \\
\bottomrule
\end{tabular}
}
  \caption{Hallucination probabilities for sentence $S_2$ - $S_5$ given there was already hallucination in previously generated sentences i.e. value in $S_3$ corresponds to the case when the third sentence is hallucinated given $S_1$ or $S_2$ is hallucinated.}
  \label{tab:conditional_probabilities_hallucinations}
\end{table}

==> Tables/hallucination_causes_further_hallucination/conditional_probabilities_not_hallucination.tex <==

% \begin{table*}[]
%     \begin{subtable}{\linewidth}
%       \centering
%         \caption{}
%         % \begin{tabular}{ll}
%         %     1 & 2
%         % \end{tabular}
%         \begin{tabular}{l|l}
%         \toprule
%         P ($S_2$ is Hallu. | $S_1$ is Hallu.) & P ($S_2$ is not Hallu. | $S_1$ is Hallu.) \\
%         \midrule
%         83.33\%                         & 16.67\%               \\
%         \bottomrule
%         \end{tabular}
%     \end{subtable}%
    
%     \begin{subtable}{\linewidth}
%       \centering
%         \caption{}
%         \begin{tabular}{l|l}
%         \toprule
%         P ($S_3$ is Hallu. | $S_2$ v $S_1$ is Hallu.) & P ($S_3$ is not Hallu. | $S_2$ v $S_1$ is Hallu.) \\
%         \midrule
%         83.33\%                         & 16.67\%               \\
%         \bottomrule
%         \end{tabular}
%     \end{subtable} 

%     \begin{subtable}{\linewidth}
%       \centering
%         \caption{}
%         \begin{tabular}{l|l}
%         \toprule
%         P ($S_4$ is Hallu. | $S_3$ v $S_2$ v $S_1$ is Hallu.) & P ($S_5$ is not Hallu. | $S_3$ v $S_2$ v $S_1$ is Hallu.) \\
%         \midrule
%         83.33\%                         & 16.67\%               \\
%         \bottomrule
%         \end{tabular}
%     \end{subtable} 
    
%     \begin{subtable}{\linewidth}
%       \centering
%         \caption{}
%         \begin{tabular}{l|l}
%         \toprule
%         P ($S_5$ is Hallu. | $S_4$ v $S_3$ v $S_2$ v $S_1$ is Hallu.) & P ($S_5$ is not Hallu. | $S_4$ v $S_3$ v $S_2$ v $S_1$ is Hallu.) \\
%         \midrule
%         83.33\%                         & 16.67\%               \\
%         \bottomrule
%         \end{tabular}
%     \end{subtable} 
%     \caption{Global caption}
    
% \end{table*}


\begin{table}[]
\centering
\small
\resizebox{0.98\linewidth}{!}
{
\begin{tabular}{l|l|l|l|l}
\toprule
 &  $\mathbf{S_2}$ & $\mathbf{S_3}$ & $\mathbf{S_4}$ & $\mathbf{S_5}$\\ \midrule
 \% Hallucinations & - & - & - & -  \\
\bottomrule
\end{tabular}
}
  \caption{Hallucination probabilities for sentence $S_2$ - $S_5$ given there was no hallucination in previously generated sentences i.e. value in $S_3$ corresponds to case when the third sentence is hallucinated given none of $S_1$ and $S_2$ is hallucinated.}
  \label{tab:conditional_probabilities_not_hallucinations}
\end{table}

==> Tables/hallucination_causes_further_hallucination/sentence_level_hallucinations.tex <==
\begin{table*}[t]
\centering
\small
\resizebox{0.98\linewidth}{!}
{
\begin{tabular}{ll|l|ll|ll|ll|lll}
\toprule
& & 
\multicolumn{2}{c}{$\mathbf{{Sentence}_2}$} &
\multicolumn{2}{c}{$\mathbf{{Sentence}_3}$} &
\multicolumn{2}{c}{$\mathbf{{Sentence}_4}$} &
\multicolumn{2}{c}{$\mathbf{{Sentence}_5}$} \\

& & Hallu & Not Hallu & Hallu & Not Hallu & Hallu & Not Hallu & Hallu & Not Hallu  \\

\midrule
\multirow{2}{*}{Prev Hallucinated}

& Count 
  & 26 & 8 & 42 & 10 & 56 & 17 & 67 & 16 \\ 

& \%
  & 76.47 & 23.53 & 80.77 & 19.23 & 76.71 & 23.29 & 80.72 & 19.28  \\ 
  

 \midrule
 \midrule
\multirow{2}{*}{Prev Not Hallucinated }


& Count & 18 & 48 & 21 & 27 & 10 & 17 & 0 & 17 \\

& \% 
& 27.27 & 72.73 & 43.75 & 56.25 & 37.04 & 62.96 & 0 & 100   \\
 % & $\mathbf{S_1}$ & $\mathbf{S_2}$ & $\mathbf{S_3}$ & $\mathbf{S_4}$ & $\mathbf{S_5}$\\ 
 % \midrule
 % \% Hallucinations & - & - & - & - & - \\
\bottomrule
\end{tabular}
}
  \caption{Sentence-level statistics of hallucinations of GPT-3 model.}
  \label{tab:sentence_level_statistics_of_hallucinations}
\end{table*}

==> Tables/uncertain_keyphrases_more_hallucination/compare_model_confidence.tex <==
\begin{table}[]
\centering
\small
% \resizebox{0.98\linewidth}{!}
{
\begin{tabular}{l|l|l}
\toprule
 &  \textbf{Hallucinated}  & \textbf{Not Hallucinated}  \\ \midrule
  Avg. Score & - & -  \\
\bottomrule
\end{tabular}
}
  \caption{Comparing Model's average score when it is hallucinated vs when it is not hallucinated.}
  \label{tab:compare_model_confidence}
\end{table}
